Neutrino Event Selection in the MicroBooNE Liquid Argon Time Projection Chamber using Wire-Cell 3-D Imaging, Clustering, and Charge-Light Matching

An accurate and efficient event reconstruction is required to realize the full scientific capability of liquid argon time projection chambers (LArTPCs). The current and future neutrino experiments that rely on massive LArTPCs create a need for new ideas and reconstruction approaches. Wire-Cell, proposed in recent years, is a novel tomographic event reconstruction method for LArTPCs. The Wire-Cell 3D imaging approach capitalizes on charge, sparsity, time, and geometry information to reconstruct a topology-agnostic 3D image of the ionization electrons prior to pattern recognition. A second novel method, the many-to-many charge-light matching, then pairs the TPC charge activity to the detected scintillation light signal, thus enabling a powerful rejection of cosmic-ray muons in the MicroBooNE detector. A robust processing of the scintillation light signal and an appropriate clustering of the reconstructed 3D image are fundamental to this technique. In this paper, we describe the principles and algorithms of these techniques and their successful application in the MicroBooNE experiment. A quantitative evaluation of the performance of these techniques is presented. Using these techniques, a 95% efficient pre-selection of neutrino charged-current events is achieved with a 30-fold reduction of non-beam-coincident cosmic-ray muons, and about 80\% of the selected neutrino charged-current events are reconstructed with at least 70% completeness and 80% purity.

==> section_matching_summary.tex <==
\subsection{Summary}\label{sec:matching_summary}
%In this section, we describe the 3D clustering techniques after the 3D imaging. 
%The presence of gaps significantly increases the challenges in clustering.
%Many advanced techniques, such as the quick convex hull, Hough transformation,
%k-d tree, principle component analysis, Kalman-filter, and various graph theory operations
%on point cloud, are used to obtain a robust result in an efficient way. 

In this section, we first described the 3D clustering techniques which follow the initial tiling, charge solving, and de-ghosting algorithms.
The challenges of gaps, coincidental overlap clusters, and separate clusters of neutrino interactions are addressed in the clustering stage. After the other clustering algorithms are applied, the de-ghosting algorithm is applied again, removing further ghosts not accessible in the first application.
Many advanced techniques, such as the quick convex hull, Hough transformation,
k-d tree, principle component analysis, Kalman filter, and various graph theory operations on point clouds
are used or referenced in the clustering algorithms. 
At this point, we introduce a robust signal processing of the scintillation light signals.
The PMT waveforms from beam discriminator and cosmic discriminator are both processed to
reconstruct flashes. 
Given the TPC clusters and PMT flashes, we explain the many-to-many charge-light matching procedures, 
which match multiple TPC clusters (charge) to the corresponding PMT flashes (light).
The many-to-many matching strategy considering all clusters (and not merely beam-coincident clusters) performs an overall optimization of the TPC-PMT pairing, boosting the ultimate performance of the matching result. 
After matching, only the in-beam flash-matched activities is considered as a potential neutrino candidate. This results in an approximately 30-fold reduction of the cosmic activities in each event.
The matching (including clustering and light reconstruction) requires significantly reduced computing resources than the imaging. 
On average, processing time is 30 seconds per event, consuming less than 1.5 GB of memory for a single CPU.

